Balanced Districting on Grid Graphs with Provable Compactness and Contiguity

Given a graph $G = (V,E)$ with vertex weights $w(v)$ and a desired number of parts $k$, the goal in graph partitioning problems is to partition the vertex set V into parts $V_1,\ldots,V_k$. Metrics for compactness, contiguity, and balance of the parts $V_i$ are frequent objectives, with much existing literature focusing on compactness and balance. Revisiting an old method known as striping, we give the first polynomial-time algorithms with guaranteed contiguity and provable bicriteria approximations for compactness and balance for planar grid graphs. We consider several types of graph partitioning, including when vertex weights vary smoothly or are stochastic, reflecting concerns in various real-world instances. We show significant improvements in experiments for balancing workloads for the fire department and reducing over-policing using 911 call data from South Fulton, GA.

==> acks.tex <==
\ACKNOWLEDGMENT{The authors gratefully acknowledge the .... }


==> annealing.tex <==
\section{Simulated Annealing}\label{sec:annealing} 

\ch{move to computations, focus on new parts (combinatorial neighborhoods) and as benchmark for comparison for computations in appendix}

To tackle the computational complexity issue in solving the mixed integer program, a commonly used alternative approach is simulated annealing (see, e.g., \cite{bertsimas1993simulated}). 
 Simulated annealing is a heuristic stochastic optimization algorithm for approximating the global optimum of a given function. The simulated annealing algorithm is based on the heuristic to explore in the neighborhood of the current solution and decide the transition randomly. Simulated annealing can achieve reasonable performance in practice for various settings, but there exist little theoretical performance guarantees. 
 In particular, in our setting, we use the current/existing partition as an initial solution. Based on this, a new solution can be founded by selecting from a set of candidate solutions. The set of candidate solutions is typically constructed as ``neighboring'' solutions to the current solution without breaking contiguity. 

Specially, for the $n$-th iteration, the simulated annealing algorithm performs the following acceptance-rejection sampling step. Suppose the starting partition is $\mathcal{P}_n$. For example, we take the existing beats plan as the starting partition in our redistricting problem. Define the set of candidate partitions as $\mathcal S_{n+1}$ and let the next proposed partition $\mathcal{P}_{n+1} \in \mathcal{S}_{n+1}$.  
The candidate partitions in $\mathcal S_{n+1}$ satisfy contiguity and balance constraints. We randomly choose one of these candidate partitions $\mathcal{P}_{n+1} \in \mathcal S_{n+1}$, and evaluate a score  
\[
    P(\mathcal{P}_{n+1}, \mathcal{P}_n|T) = 
    \begin{cases}
    1, & Z(\mathcal{P}_{n+1}) < Z(\mathcal{P}_n),\\
    \exp\{|Z(\mathcal{P}_{n
    +1}) - Z(\mathcal{P}_n)|/T\}, & \text{otherwise}.\\
    \end{cases}
\] 
where $Z(\cdot)$ denotes the cost function value associated with the partition (e.g., the compactness shown in \eqref{eq:compactness}), $T$ is a preset temperature that determines the speed of convergence, and the $P$ is the acceptance probability. Generate an independent uniform random variable $U \in [0, 1]$. The proposed partition is accepted if  $P(\mathcal{P}_{n+1}, \mathcal{P}_n|T) \ge U$. Note that in simulated annealing, there is a chance for the transition to happen from a ``low-cost'' partition to a ``high-cost'' partition, which may prevent the algorithm being trapped locally and finding a sub-optimal partition. 
%
% The last accepted candidate design will be considered as the refined beat design based on the greedy design. Figure ~\ref{fig:beat-design} shows the refined 15-beat design based on 15-beat greedy design using simulated annealing
%
The choice of the set candidate partitions $\mathcal S_{n+1}$ is critical for the performance of simulated annealing, and it involves the trade-off between exploration and exploitation. Now we introduce two strategies in search of ``neighboring'' partitions. 

\paragraph{One-swapping neighborhoods.}

As illustrated in Figure~\ref{fig:sa-demo} (a), we first consider the following simple heuristic in constructing the candidate set. This allows us to search for local optimal partitions at a reasonable computational cost~\cite{Wang2013}. The candidate set is constructed as the set that contains all partitions swapping a single vertex assignments at the boundaries of the current partition. This simple heuristic is easy to implement, since the number of candidate partitions is usually small (since we only swap one end of boundary edge); however, since the change of partition in each iteration is too minuscule to sufficiently explore its neighborhoods, we may still be easily trapped at a small local neighborhood and converging to a locally optimal partition.

\paragraph{Combinatorial neighborhoods.}

\begin{figure}[!t]
\centering
% {\footnotesize
\begin{subfigure}[h]{0.9\linewidth}
\includegraphics[width=\linewidth]{imgs/sa-demo-v1.pdf}
\caption{One-swapping neighborhoods}
\vfill
\vspace{0.1in}
\end{subfigure}
\begin{subfigure}[h]{0.9\linewidth}
\includegraphics[width=\linewidth]{imgs/sa-demo-v2.pdf}
\caption{Combinatorial neighborhoods.}
\end{subfigure}
\caption{An illustration of one-swapping neighborhoods and combinatorial neighborhoods. Red and blue boxes represent vertices in different parts. Thick black line represents the boundary of two parts. Left figure shows the current partition $\mathcal{P}_n$; middle and right figures show the candidate partition sets for the next iteration $\mathcal{S}_{n+1}$.}
% }
\label{fig:sa-demo}
\end{figure}

We further explore a combinatorial method to increase the set of candidate set $\mathcal S_{n+1}$ as demonstrated in Figure~\ref{fig:sa-demo} (b). These combinatorial neighborhoods are found by shifting the current partition with multiple swappings of vertices assignments in place of one-swapping strategy. This helps create a larger set of candidate solutions, rather than a small neighborhood as in the first heuristic. In practice, we have shown that this combinatorial strategy is more efficient in search of compact partitions than one-swapping strategy, which will be further discussed in Section~\ref{sec:computations}. 

%\subsection{Adaptations for Stochastic Weights}

%\sg{Changes for the stochastic setting with smooth weights assumption.}



==> roughtnotes.tex <==
\iffalse 
\begin{algorithm}[t]\footnotesize
 \caption{The general dynamic path algorithm with weights}
 \begin{algorithmic}[1]
\State \textbf{Input:} Graph $G=(V,E)$ with vertex set $V$, and vertex weights $w(v)$; desired number of parts $k\in \mathbb{N}$; balance parameter $\varepsilon>0$.
\State \textbf{Output:} A partition of the vertex set into $k$ connected parts, with each part having total weight within $\varepsilon$ fraction of the average weight $A=\frac{\sum_{v\in V}w(v)}{k}$. 
\State Find an ordering $v_1,\dots,v_n$ of $V$, using the striping technique discussed below.
\State Apply Algorithm~\ref{alg:dynamic_striping} with ordering $v_1,\dots,v_n$. 
\Return The resulting partition.
\end{algorithmic}
\label{alg:master_dynamic}
\end{algorithm}\fi 


